Speech Token Prediction via Compressed-to-fine Language Modeling for Speech Generation

Neural audio codecs, used as speech tokenizers, have demonstrated remarkable potential in the field of speech generation. However, to ensure high-fidelity audio reconstruction, neural audio codecs typically encode audio into long sequences of speech tokens, posing a significant challenge for downstream language models in long-context modeling. We observe that speech token sequences exhibit short-range dependency: due to the monotonic alignment between text and speech in text-to-speech (TTS) tasks, the prediction of the current token primarily relies on its local context, while long-range tokens contribute less to the current token prediction and often contain redundant information. Inspired by this observation, we propose a \textbf{compressed-to-fine language modeling} approach to address the challenge of long sequence speech tokens within neural codec language models: (1) \textbf{Fine-grained Initial and Short-range Information}: Our approach retains the prompt and local tokens during prediction to ensure text alignment and the integrity of paralinguistic information; (2) \textbf{Compressed Long-range Context}: Our approach compresses long-range token spans into compact representations to reduce redundant information while preserving essential semantics. Extensive experiments on various neural audio codecs and downstream language models validate the effectiveness and generalizability of the proposed approach, highlighting the importance of token compression in improving speech generation within neural codec language models. The demo of audio samples will be available at https://anonymous.4open.science/r/SpeechTokenPredictionViaCompressedToFinedLM.

==> section/4_exp_0409.tex <==
% the subscripts (e.g., $330M, 44Kh$) denote the model size and data scale.
\begin{table*}[!t]
    \centering
    \caption{The speech generation results on LibriTTS test set. \textbf{Bold} means the best result, and \underline{underline} means the second-best result. The superscripts \textit{CF} and \textit{vanilla} are short for \textit{compressed-to-fine language modeling} and \textit{the original implementation of VALL-E}. $\dagger$ indicates the result is cited from the original paper. \wen{(1) Please note that captions of all tables and figures should be relatively self-contained, that is, they include information of the task, test sets, evaluation metrics, and important information, such as how the results are obtained: cited from original papers, evaluate the open-sourced model on the test sets by us, the model is reimplemented and evaluated by us. For example, it is not clear how the results of USLM, VoiceCraft etc are obtained. (2) Please explain Scale, it seems to include the model size and training data size of neural codec LM, then please complete the model size info for all baselines. (3) I added a separator, it would help to clarify the first group and second group, and that we compared CF to the baseline for the neural codecs and neural codec LMs in the second group. Maybe we could consider grouping the neural codes into single-codebook and multi-codebook. Also, it is most important to show that for each configuration of neural codec + neural codec LM, CF always outperforms the baseline, hence boldfacing the best value for each metric across all model configurations is a bit odd.}
    }
    \scalebox{0.95}{
    \begin{tabular}{cc|lc|ccc}
    \toprule
        \multirow{2}{*}{\makecell[c]{Neural\\Audio Codec}} & \multirow{2}{*}{Bandwidth} & \multirow{2}{*}{\makecell[c]{Neural Codec\\ Language Model}} & \multirow{2}{*}{Scale} & \multicolumn{3}{c}{Objective} \\ 
         & & & & WER↓ & SIM↑ & UTMOS↑ \\ \midrule
        Ground Truth & - & - & - & - & 69.72\% & 4.15 \\ 
    \midrule
        % mHuBERT~\cite{hubert} & 0.5 kbps & SpeechGPT~\cite{speechgpt} & 72Kh & 13.39 & - & 4.15 \\ \midrule
        \multirow{2}{*}{EnCodec~\cite{encodec}} & \multirow{2}{*}{2.2 kbps} & \multirow{2}{*}{VoiceCraft~\cite{voicecraft}} & 330M,9Kh & 4.46 & 52.15\% & 3.55 \\ 
         &  &  & 830M,9Kh & 3.31 & 56.75\% & 3.78 \\ 
    \midrule
        Mel VQ-VAE & - & XTTS\_v2~\cite{xtts} & 27Kh & 2.98 & \underline{59.14\%} & 3.94 \\ 
    \midrule
        \multirow{1}{*}{SpeechTokenizer~\cite{speechtokenizer}} & \multirow{1}{*}{4.0 kbps} & USLM~\cite{speechtokenizer} & 960h & 6.25 & 56.93\% & 3.12 \\ 
        % &  & AnyGPT~\cite{anygpt} & 57Kh & 25.75 & 25.66\% & 3.19 \\ 
        % &  & VALL-E$_{960h}$ & 14.32 & 48.90\% & 3.87 \\ 
    \midrule
        \multirow{2}{*}{EnCodec~\cite{encodec}} & \multirow{2}{*}{6.0 kbps} & VALL-E^{\dagger}~\cite{valle} & 60Kh & 5.90 & 58.00\% & - \\  
        &  & VALL-E R^{\dagger}~\cite{valler} & 960h & 3.18 & - & - \\
    \midrule
    \midrule
        \multirow{2}{*}{HuBERT~\cite{hubert}} & \multirow{2}{*}{0.5 kbps} & decoder-only & \multirow{2}{*}{960h} & 7.04 & - & 4.07 \\ % [0.10cm]
        &  & decoder-only^{\text{CF}} &  & 5.86 & - & 4.08 \\
    \midrule
        \multirow{2}{*}{BigCodec~\cite{bigcodec}} & \multirow{2}{*}{1.04 kbps} & decoder-only & \multirow{2}{*}{960h} & 16.58 & 46.04\% & 3.78 \\ % [0.10cm]
        &  & decoder-only^{\text{CF}} &  & 10.90 & 46.51\% & 4.01 \\
    \midrule
        \multirow{2}{*}{WavTokenizer~\cite{wavtokenizer}} & \multirow{2}{*}{0.9 kbps} & decoder-only & \multirow{2}{*}{960h} & 5.94 & 47.59\% & 4.14 \\ % [0.10cm]
        &  & decoder-only^{\text{CF}} &  & 3.40 & 47.99\% & \textbf{4.19} \\
    \midrule
        \multirow{3}{*}{EnCodec~\cite{funcodec}} & \multirow{3}{*}{4.0 kbps} & VALL-E^{\text{vanilla}} & \multirow{3}{*}{960h} & 7.59 & 56.08\% & 4.13 \\ % [0.10cm]
        & & VALL-E & & 5.23 & 56.64\% & 4.16 \\ % [0.10cm]
        &  & VALL-E^{\text{CF}} & & \textbf{2.36} & \textbf{59.75\%} & \underline{4.18} \\ \midrule
        \multirow{2}{*}{EnCodec~\cite{funcodec}} & \multirow{2}{*}{4.0 kbps} & VALL-E & \multirow{2}{*}{20Kh} & 5.05 & 53.66\% & 4.09 \\ % [0.10cm]
        &  & VALL-E^{\text{CF}} & & \underline{2.21} & 57.72\% & 4.15 \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-0.68cm}
    \label{tab:tts}
\end{table*}


\begin{table}[!t]
    \centering
    \caption{Subjective performance on LibriTTS test set. }
    \scalebox{0.92}{
    \begin{tabular}{c|l|ccc}
    \toprule
        \multirow{2}{*}{\makecell[c]{Neural\\Audio Codec}} & \multirow{2}{*}{\makecell[c]{Neural Codec\\ Language Model}} & \multicolumn{3}{c}{Subjective} \\ 
         & & MOS↑ & SMOS↑ & PMOS↑ \\ \midrule
        Ground Truth & - & 4.43 & 4.23 & 4.12 \\ 
    \midrule
        \multirow{2}{*}{HuBERT~\cite{hubert}} & decoder-only & 3.51 & - & 3.79 \\ 
        &  decoder-only^{\text{CF}} & 3.67 & - & 3.75 \\
    \midrule
        \multirow{2}{*}{WavTokenizer~\cite{wavtokenizer}} & decoder-only & 3.86 & 3.37 & 3.59 \\ 
        &  decoder-only^{\text{CF}} & 3.92 & 3.43 & 3.61 \\
    \midrule
        \multirow{2}{*}{EnCodec~\cite{funcodec}} & VALL-E & 3.98 & 3.49 & 3.81 \\ 
        & VALL-E^{\text{CF}} & 4.01 & 3.62 & 3.90 \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-0.68cm}
    \label{tab:tts_subjective}
\end{table}




\subsection{Model Setup} 
We conduct experiments based on various neural audio codecs, categorized into multi-codebook and single-codebook codecs.\wen{Please note that it is important to explain the rationale of baseline selection, in our case, why did we choose these certain multi-codebook and single-codebook codecs to evaluate our proposed approach?} 

\textbf{Multi-codebook}. We train EnCodec~\cite{encodec} (8 codebooks, each with 1024 codewords, reproduced by FunCodec~\cite{funcodec}) and VALL-E~\cite{valle} on LibriTTS~\cite{libritts}. EnCodec is optimized by the Adam optimizer~\cite{2014adam} with an initial learning rate of 3e-4. Audio samples are truncated to 1.28 seconds, resampled to 16 kHz, with a batch size of 384. We optimize VALL-E by the AdamW optimizer with an initial learning rate of 0.01~\cite{xcodec} and beta parameters (0.5, 0.9).

\textbf{Single-codebook}. We use pre-trained HuBERT~\cite{hubert} and its corresponding unit-based HiFiGAN~\cite{hifigan}, WavTokenizer~\cite{wavtokenizer}, and BigCodec~\cite{bigcodec} as speech tokenizers. The decoder-only transformer is adopted as the neural codec language model, and trained on LibriTTS, using the AdamW optimizer with an initial learning rate of 9.5e-5 and beta parameters (0.5, 0.9).
% \qian{0.000095 -> 9.5e-5}

\textbf{Transformer architecture}. All transformer models in both VALL-E and decoder-only architecture have a dimension of 1024, 12 transformer blocks, and 16 attention heads. To improve the performance, we incorporate several components from the Llama model~\cite{2023llama} into the transformer block, including RoPE and the SiLU activation function. We denote the original implemented VALL-E by \textbf{VALL-E$^{\text{vanilla}}$}, and the improved version of VALL-E by \textbf{VALL-E}.\wen{I would suggest we denote the improver version of VALL-E with an indicator, instead of VALL-E, such as VALL-E$^*$.}

% Additionally, to enhance training stability, we replace the adaptive layer norm in the original VALL-E model with additive layer embeddings to indicate different non-autoregressive transformer layers. 

~\cite{guo2025recent, cho2024sylber, syllablelm} suggest that 5Hz discrete units can effectively align with syllables\wen{Just curious, how does this statement hold across a wide range of languages?}\WRC{Previous research only focuses on English and LibriSpeech, other language and modality of audio (e.g., sound, music) have not been explored.}, capturing essential linguistic structure. Thus, we set the compression rate $\text{CR} = 5$ to compress the speech tokens of a 1-second span into 5 compact representations, which retain coarse-grained semantic information. Detailed hyperparameters of compressed-to-fine language modeling are listed in Table~\ref{tab:cf_setup}.\wen{Since this table of hyperparameters appears first, it should appear first, hence as Table 1.}

\begin{table}[h]
    \centering
    \caption{Details of compressed-to-fine language modeling across various neural audio codecs and neural codec language models. The symbol "-" indicates that $N_{\text{NAR}}$ is not used.}
    \scalebox{0.78}{
    \begin{tabular}{ccc|c|ccc|c}
    \toprule
        \multirow{2}{*}{\makecell[c]{Neural\\Audio Codec}} & \multirow{2}{*}{\makecell[c]{sampling\\rate}} & \multirow{2}{*}{\makecell[c]{frame\\rate}} & \multirow{2}{*}{\makecell[c]{Neural Codec\\ Language Model}} & \multicolumn{3}{c|}{$\text{LM}_{\text{AR}}$} & $\text{LM}_{\text{NAR}}$ \\ \cline{5-8}
         &  &  & & $G$ & CR & $N_{\text{AR}}$ & $N_{\text{NAR}}$ \\ \midrule
        HuBERT & 16000 & 50Hz & decoder-only & 10 & 5 & 50 & - \\ \bottomrule
        BigCodec & 16000 & 80Hz & decoder-only & 16 & 5 & 80 & - \\ \bottomrule
        WavTokenizer & 24000 & 75Hz & decoder-only & 15 & 5 & 75 & - \\ \midrule
        EnCodec & 16000 & 50Hz & VALL-E & 10 & 5 & 50 & 50 \\ \bottomrule
    \end{tabular}}
    \label{tab:cf_setup}
\end{table}

\subsection{Baselines}
For speech generation, we employ various neural codec language models as baselines, including VoiceCraft~\cite{voicecraft}, SpeechTokenizer-based USLM~\cite{speechtokenizer} and XTTS v2~\cite{xtts}.\wen{Similarly, please explain the rationale of selecting these neural codec language models as baselines.}

Considering that VALL-E~\cite{valle} and VALL-E R~\cite{valler} do not provide reproducible code, we cite the test results from their original papers. Since they employ different models to evaluate SIM (speaker similarity)\wen{please spell out} scores, which differ significantly from other baseline models, we report only part of SIM results to ensure fairness. The results of zero-shot speech generation are shown in Table~\ref{tab:tts}.\wen{This paragraph about how the results in table are obtained should be included in the discussion of experimental results, not here.}


% maskgct, mars6

\subsection{Datasets}
We train neural codec language models using LibriTTS~\cite{libritts} (960 hours), validating performance with its test set for speech generation. To assess data scaling, we expand the training data to 44,000 hours by adding MLS~\cite{MLS} dataset.
\wen{You could merge Section 4.1, 4.2, 4.3 as the baseline neural codecs and neural codec language models and describe how they are trained.}

\subsection{Evaluation Metrics}

\textbf{Objective evaluation.} Whisper~\cite{whisper} model is used to transcribe the generated speech and then calculate WER (Word Error Rate). To evaluate SIM (speaker similarity), we use 3D-speaker~\cite{3dspeaker} toolkit to extract speaker embeddings from the generated speech and reference speech, and compute the cosine similarity between the normalized embeddings. UTMOS~\cite{utmos} also serves as an automatic Mean Opinion Score (MOS) prediction system to assess the naturalness of the generated speech. 

RTF (Real-Time Factor) is defined as the ratio of the time required to generate speech to the duration of the generated speech. A lower RTF value indicates faster speech generation.

\textbf{Subjective evaluation.} We randomly select speech samples from the LibriTTS~\cite{libritts} test set to conduct MOS~\cite{chu2006objective}, Similarity Mean Opinion Score (SMOS)~\citep{chu2006objective} and Prosody MOS (PMOS) evaluations. MOS assesses the naturalness of the generated speech, SMOS measures the timbre similarity between the generated speech and voice of the original speaker, and PMOS evaluates the prosody of the generated speech.


